Improve Event Extraction via Self-Training with Gradient Guidance

Data scarcity has been the main factor that hinders the progress of event extraction. To overcome this issue, we propose a Self-Training with Feedback (STF) framework that leverages the large-scale unlabeled data and acquires feedback for each new event prediction from the unlabeled data by comparing it to the Abstract Meaning Representation (AMR) graph of the same sentence. Specifically, STF consists of (1) a base event extraction model trained on existing event annotations and then applied to large-scale unlabeled corpora to predict new event mentions as pseudo training samples, and (2) a novel scoring model that takes in each new predicted event trigger, an argument, its argument role, as well as their paths in the AMR graph to estimate a compatibility score indicating the correctness of the pseudo label. The compatibility scores further act as feedback to encourage or discourage the model learning on the pseudo labels during self-training. Experimental results on three benchmark datasets, including ACE05-E, ACE05-E+, and ERE, demonstrate the effectiveness of the STF framework on event extraction, especially event argument extraction, with significant performance gain over the base event extraction models and strong baselines. Our experimental analysis further shows that STF is a generic framework as it can be applied to improve most, if not all, event extraction models by leveraging large-scale unlabeled data, even when high-quality AMR graph annotations are not available.

==> 1introduction_bak.tex <==
\section{Introduction}
\lifu{change the }
Event extraction (EE), which aims to identify and classify event triggers and arguments, has been a long challenging problem in natural language processing. Despite the large performance leap brought by advances in deep learning, recent studies \cite{deng2021ontoed, maven, CLEVE} have shown that the data scarcity of existing event annotations have been the major issues that hinder the progress of EE.
However, creating event annotations is extremely time consuming and complicated, e.g., it takes several linguists over one year to annotate 500 documents for ACE05 which merely contains 4,202 event annotations in the training set and 450 in the development set. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/gradient_fix.pdf}
    \caption{The star is the global optimal point. The black lines show the gradients $g_1$ and $g_2$ compute on the pseudo event labels and the green lines show the gradients after multiplying the compatibility scores. The red dash is a vector addition of $g_1$ and $g_2$ and the green dash line is the vector addition of the fixed gradients.}
    \label{fig:fix_gradient}
\end{figure}
To overcome this issue, one line of works~\cite{automatically_label_ee_chen2017, automatically_label_ee_zeng2018, automatically_label_ee_jun2018, automatically_label_ee_wang2019} develop automatic methods to generate additional training data. The generation process often involves complicated human-written rules, incomplete knowledge bases and additional linguistic knowledge. Those systems suffer from inevitable noises in the generation process and errors can easily accumulate throughout the generation steps.
% Another line of works propose to leverage the sentence semantic structures as additional features to provide more information to the model. \cite{amr_ie_xiang2015} is the first to leverage AMR graph as additional linguistic features to performance Event Detection. \cite{huang2016liberal} leverages the AMR graph to identify the set of candidate arguments given a trigger in the Liberal Event Extraction setting and clearly show a subset of fine-grained AMR semantic relations are informative for inferring argument roles. \cite{amr_ie_sudha2017} verifies event structure can be a subgraph of an AMR graph and a neural network can identify the event subgraph given its corresponsing AMR graph. In addition, it shows the pattern on the shortest path between two event node in the AMR graph can be used to filter out noise distant-labeled argument roles. \cite{huang2018zero} perform zero-shot event extraction by grounding the AMR structure to the target event ontology. CLEVE~\cite{CLEVE} propose an AMR subgraph discrimination objective for event structure pre-training. The graph encoder learns to encode rich semantic structure knowledge which can benefit downstream tasks. AMR-IE~\cite{AMR_IE} and BERT-AMR-KG~\cite{zixuan_bio_amr} enable the candidate arguments and event triggers to aggregate neighborhood information from surrounding nodes in the AMR graph. However, all of the methods mentioned above require AMR graph at inference time as input features which makes the overall model highly depend on the AMR parser and can easily overfits to the noisy AMR graph.
Another line of works propose to leverage the Abstract Meaning Representations as additional features to provide more information to the model. The coherence between AMR Path and Argument Role can be easily spotted in the following examples where the red tokens denote arguments and blue tokens denote event triggers:
\begin{itemize}
  \item The Apache troop opened its tank \textcolor{red}{guns}, opened its own mortars, decimated that unit, put it out of existence and probably \textcolor{blue}{killed} some 20 Iraqis in the process. \\AMR Path: [\textcolor{blue}{killed}, ARG0, troop, MEDIUM, \textcolor{red}{guns}] \\Argument Role: Instrument
  \item The Iraqi \textcolor{red}{unit} in possession of those guns \textcolor{blue}{fired} mortars in the direction of the 7th Cavalry. \\ AMR Path: [\textcolor{blue}{fired}, ARG0, \textcolor{red}{unit}] \\ Argument Role: Attacker
  \item U.S.-led forces were able to press farther north after \textcolor{blue}{defeating} Iraqi Republican Guard units at Karbala and \textcolor{red}{Kut}. \\ AMR Path: [\textcolor{blue}{defeating}, PLACE, and, OPTION, \textcolor{red}{Kut}] \\ Argument Role: Place
\end{itemize}
\cite{amr_ie_xiang2015} input serialized AMR graph as additional linguistic features to performance Event Detection. \cite{huang2016liberal,amr_ie_sudha2017,huang2018zero} translate AMR graphs into event structures. \cite{AMR_IE,zixuan_bio_amr} learn better candidate argument and event trigger representations by aggregating neighborhood information from their surrounding nodes in the AMR graph. However, all methods mentioned above require AMR graph at inference time as input which makes the overall model highly depend on the AMR parser and can easily overfits to the noisy AMR graph. 


In this work, we propose \selftraininggg{} (\stgg{}), a \selftraining{} framework that can both address data scarcity and leverage AMR graph without requiring it at test time. 
\selftraining{} allows the trained model to learn further by regarding its own prediction as a pseudo labels on large-scale unlabeled corpus and has shown promising performance in many NLP tasks. However, simply adding high-confidence predictions to the training set can introduce noises~\cite{gradual_drift_ner, confirmation_bias, mentor_net}, especially given that the current state-of-the-art performance of event argument extraction is still less than 59\% F1. \cite{amr_ie_sudha2017} show that the coherence between AMR and EE annotations can be used to filter out noisy pseudo event labels. Inspired by them, we propose to a novel scoring model that can measure the compatibility between pseudo event labels and AMR annotations and compute compatibility scores ranging in [-1,1]. The theoretical justification of this idea roots in policy gradient~\cite{reinforce,policy_gradient} and pseudo-label reweighting~\cite{pseudo_label_reweight}. As shown in Fig~\ref{fig:fix_gradient}, the compatibility scores can fix the direction and magnitude of the gradients computed on the pseudo event labels. In addition, we find that model selected by the development set can be highly biased due to its small size and lack of multiple event and argument role types. We propose a novel model selection method by measuring the the compatibility scores of the model's predictions on some large-scale held out unlabeled data.
To examine the effect of our proposed approach, we train \stgg{} on AMR 3.0\footnote{https://catalog.ldc.upenn.edu/LDC2020T02.} and the AMR predictions on New York Times (NYT)\footnote{https://catalog.ldc.upenn.edu/LDC2008T19} corpus as additional unlabeled data, and evaluate the event extraction performance on three public benchmark datasets: \ace{}\footnote{https://catalog.ldc.upenn.edu/LDC2006T06}, \aceplus{}\footnote{https://catalog.ldc.upenn.edu/LDC2006T06}, and \ere{}\footnote{Deep Exploration and Filtering of
Test (DEFT) program.}. The experimental results demonstrate that: (1) \selftraining{} alone barely improves event extraction due to the noise introduced by the pseudo examples, while the proposed \stgg{} framework makes robust and efficient use of such pseudo examples;
(2) \stgg{} can be applied to improve most, if not all, of the event extraction models and achieves the new state of the art on the three public benchmark datasets; (3) By exploiting different unlabeled corpora with gold or system-based AMR parsing, \stgg{} always improves the base event extraction models, demonstrating that it is less sensitive to the quality of AMR parsing; (4) The proposed model selection method is less biased and does not require any labeled data.
(4)--> (1)
We learn to estimate the quality of the IE prediction by learning to measure coherence between IE prediction and AMR prediction. .....we contribute ...
(1) (mention the quality estimator),(2),(3) 
(4) By utilizing the proposed quality estimator, we show that we can perform better model selection, resolving the label distribution mismatch problem between train, validation and test.

==> backups/3approach_backup.tex <==
\section{Event Extraction}
\zhiyang{define the output space as in $(\tau_i, \alpha_{i,j}, \epsilon_j)$, draw a figure of general event extraction model and show the input trigger, role . in the identification step, we identify the span of event trigger and span of arguments in X. }
The event extraction task consists of three subtasks: event detection, argument identification and argument role classification. Given an input sentence $W=[w_1, w_2, ... ,w_N]$, event detection aims to identify the span of an event trigger $\tau_i$ from $W$ and assign label $l^t_i$ to the trigger from a set of predefined event types $\mathcal{L}^t$. Argument identification aims to find the span of an argument $\varepsilon_j$ in $W$, and argument role classification further predicts the role $\alpha_{i,j}$ of an argument $\varepsilon_j$ in an event $\tau_i$ given a set of predefined argument roles $\mathcal{L}^a$.

\begin{table}[ht!]
%\setlength\tabcolsep{4pt}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ l | r |  }
\toprule
Symbol &   \\
\midrule
% Gradient \\
$w_i$ & a single token \\
$W$ & token sequence   \\
$\tau_i$ & event trigger \\
$t_i$ & event trigger type \\
$L^t$ & all event trigger types \\
$\varepsilon_j$ & argument \\
$\alpha_{i,j}$ & argument role type \\
$L^a$ & all argument role types \\
$\mat{X}$ & sequence of word representations \\
$\vvv{x}_i$ & single word representation \\
$\mat{W}^{tri\_i}$ & linear layer for trigger identification \\
$\widehat{\mat{Y}}^{tri\_i}$ & sequence of predicted score vectors for event types\\
% $\hat{\vvv{y}}^{tri\_i}_i$ & predicted score vector of event types for a single token \\
$A$ & transition matrix for event types \\
$\vvv{y}^{tri\_i}$ & ground truth trigger type vector for the sequence \\
$L^I()$ & the event type identification loss \\
$(m,n)$ & the event trigger span \\
$(p,q)$ & the argument span \\
$\mat{W}^{tri\_c}$ & linear layer for trigger classification \\
$\mat{Y}^{tri\_c}$ & ground-truth event trigger labels  \\
$\vvv{y}^{tri\_c}_i$ & ground-truth event trigger label for ith trigger  \\
$\hat{\vvv{y}}^{tri\_c}_i$ & predicted event trigger label for ith trigger  \\
$\mat{W}^{arg\_c}$ & linear layer for argument role classification \\
$\mat{Y}^{arg\_c}$ & ground-truth argument role labels  \\
$\vvv{y}^{arg\_c}_{i,j}$ & ground-truth argument role label for (ith trigger, jth argument)  \\
$\hat{\vvv{y}}^{arg\_c}_{i,j}$ & ground-truth argument role label for (ith trigger, jth argument)  \\
$\mathrm{V}^{tri}$ & set of event triggers \\
$\mathrm{E}^{role}$ & set of (event and argument) pairs \\
$\mathcal{L}^C()$ & the event type identification loss \\
$G^e$ & information extraction graph \\
$\hat{G}^e$ & predicted information extraction graph \\
$\vvv{u}$ &weight of global feature vector\\
$f^{global()}$ &global feature vector\\
$\mathcal{L}^E()$ & the combined loss for OneIE \\

\bottomrule
\end{tabular}
}
\end{center}
\vspace{-0.4cm}
\caption{
}
\label{tab:notation}
\end{table}

\subsection{Base Event Extraction Model}
OneIE \cite{OneIE} is a unified model that jointly performs event, entity extractions and relation classification. Although, entity extraction and relation classification are not part of the event extraction task, the interaction between three tasks can benefit all of them and achieve better performance~\cite{OneIE,FourIE}. Thus, to show the proposed framework can improve upon the state of the art model, we select OneIE as our base event extraction model. OneIE performs event extraction in four steps: (1) The \textbf{language encoder}~\cite{bert, roberta} encodes the input sentence $W$ into contextualized word representations $\mat{X}=[\vvv{x}_1, \vvv{x}_2, ... ,\vvv{x}_N]$\footnote{We use bold symbols to denote vector representations, and capital bold symbols to denote matrix.}. 
% (2) Two \textbf{identification layers}, one identifies the spans of event triggers and one identifies the spans of arguments in \mat{X}. 
% both of them take in the contextualized word representations $\mat{X}$ and one computes the score vector $\hat{\vvv{y}}^{tri\_i}_i$ of event types for each token $\vvv{x}_i$ and one computes the score vector $\hat{\vvv{y}}^{arg\_i}_i$ of arguments for each token $\vvv{x}_i$. 
(2) Two \textbf{identification layers} respectively identifies the spans of event triggers and the spans of arguments in \mat{X}.
Two identification layers have the same architectures. For simplicity, we only explain the identification layer for event triggers\footnote{We explain the identification layer for arguments in appendix.}. 
% The identification layer utilizes BIO tags and CRF layers~\cite{crf} to compute the probability of the ground-truth label sequence $\vvv{y}^\ast$.
Given $\mat{X}$, the identification layer computes the score vectors of event types for the sequence as $\widehat{\mat{Y}}^{tri\_i}=Softmax(\mat{W}^{tri\_i}^\top\mat{X})$. Then $\widehat{\mat{Y}}^{tri\_i}\in R^{N\times |L^t|}$ is passed into a CRF layer~\cite{crf} to compute the score for the ground-truth label sequence $\vvv{y}^{tri\_i}\in R^N$. 
% \begin{align*}
% S(\vvv{y}^{tri\_i})=\sum_{i=1}^{N}{\widehat{\mat{Y}}^{tri\_i}_{i,\vvv{y}^{tri\_i}_i}+\sum_{i=1}^{N-1}\mat{A}_{\vvv{y}^{tri\_i}_i,\vvv{y}^{tri\_i}_{i+1}}},
% \end{align*}
\begin{align*}
S(\vvv{y}^{tri\_i})=\sum_{i=1}^{N}{\widehat{\mat{Y}}^{tri\_i}_{i,\vvv{y}^{tri\_i}_i}+\sum_{i=1}^{N-1}\mat{A}_{\vvv{y}^{tri\_i}_i,\vvv{y}^{tri\_i}_{i+1}}},
\end{align*}
$\mat{A}\in R^{|L^t|\times |L^t|}$ denotes the transition matrix which learns the transition scores between event types. The objective for the identification layer is the negative log-likelihood of the ground-truth label sequence:  
\begin{align*}
\mathcal{L}^I(\hat{\vvv{y}}^{tri\_i})=-S(\hat{\vvv{y}}^{tri\_i})+\log{\sum_{\vvv{y}\in{\widehat{\mat{Y}}^{tri\_i}}}\exp{S({\vvv{y}})}},
\end{align*}
Although, the identification layer for event triggers can classify the event types, OneIE only considers the spans and ignores the labels. Given the identified span for an event trigger $\tau_i$ or an argument $\varepsilon_j$, the representation of $\tau_i$ or $\varepsilon_j$ is computed by averaging the token representations in $\mat{X}$ across the identified span. For example, for an event trigger $\tau_i$ with span $(m, n)$, the representation of $\tau_i$ is $\frac{1}{n-m}\sum_{i=m}^{n}{\vvv{x}_i}$ and for an argument $\varepsilon_j$ with span $(p, q)$, the representation of $\varepsilon_j$ is $\frac{1}{q-p}\sum_{i=p}^{q}{\vvv{x}_i}$. 
(3) Two\footnote{We defer the description of entity classification and relation classification layers to Appendix ref(), since they are not part of the event extraction task.} \textbf{classification layers}, one takes in an event trigger representation and classifies the event trigger type, and one takes in the concatenated event trigger and argument representation and classifies the argument role type. Specifically, the score vector of event types for an event trigger $\tau_i$ is computed as $\hat{\vvv{y}}^{tri\_c}_i=Softmax\left(\mat{W}^{tri\_c}^\top(\frac{1}{n-m}\sum_{i=m}^{n}{\vvv{x}_i})\right)$. The score vector of the argument role types for an event $\tau_i$ and argument $\varepsilon_j$ pair is computed as $\hat{\vvv{y}}^{arg\_c}_i=Softmax\left(\mat{W}^{arg\_c}^\top[\frac{1}{n-m}\sum_{i=m}^{n}{\vvv{x}_i},\frac{1}{q-p}\sum_{j=p}^{q}{\vvv{x}_j}]\right)$. 
Given the set of ground-truth labels $\mat{y}^{tri\_c}\in [0,1]^{|\mathrm{V}^{tri}|\times |L^t|}$ for the set of event triggers $\tau_i\in\mathrm{V}^{tri}$ and the ground-truth labels $\mat{y}^{arg\_c}\in R^{|\mathrm{E}^{role}|\times|L^a|}$ for the set of event and argument pairs $(\tau_i, \varepsilon_j)\in\mathrm{E}^{role}$, the objective is to minimize the cross-entropy loss:
\begin{align*}
\mathcal{L}^C(\mat{y}^{tri\_c},\mat{y}^{arg\_c})=-\sum_i\vvv{y}^{tri\_c}_i \log{\hat{\vvv{y}}^{tri\_c}_i}\\-
\sum_i\sum_j\vvv{y}^{arg\_c}_{i,j} \log{\hat{\vvv{y}}^{arg\_c}_{i,j}},
\end{align*}
(4) After computing the score vectors for event triggers, entities, relations and argument roles, OneIE does not simply take the labels with maximum scores as the final predictions. The labels between each task have constraints which is defined as Sub-tasks interaction in OneIE. For example, in an 'Attack' event, the argument with a 'Location' entity type is unlike to have an 'Attacker' role. Simply taking the argmax labels can cause conflicts. In addition, OneIE defines Crossinstance interactions between events. For example, the 'Defendant' in an 'Sentence' event can also be an 'Agent' in a 'Die' event. Thus, to capture two interactions, OneIE proposes a global feature template $f^{global}()$ in which each entry specifies a case of interaction. One can think the predictions from OneIE organize a graph $G^e$ (event triggers and arguments are nodes and relations and argument roles are edges), and the value for each entry in the global features is collected from the graph $f^{global}(G^e)$. During training, a weight vector $\vvv{u}$ is learned to assign weights to global features and the global feature score for $G^e$ is computed as $\vvv{u}\cdot f^{global}(G^e)$. The objective is to promote the ground-truth graph have the highest score. Thus, the training objective is defined as:
\begin{align*}
\mathcal{L}^G(G^e)=\vvv{u}f^{global}(\hat{G}^e)-\vvv{u}f^{global}(G^e),
\end{align*}
where $\hat{G}^e$ is the predicted local optimal graph.
% OneIE \cite{OneIE} jointly extracts entities, relations and events from each single sentence. It has four components: First, a language model encoder \citep{bert,roberta} computes the contextualized word representations $\mat{W}=[\vvv{w}_1, \vvv{w}_2, ... ,\vvv{w}_N]$\footnote{We use bold symbols to denote vector representations.} from an input sequence $W$. Then, two local classifiers $\textsl{FFN}^I$s with CRF layers~\citep{crf} are trained to identify the spans of events and arguments respectively. The sequence of score vectors for all labels is $\mat{Y}=Softmax(\textsl{FFN}^I(\mat{W}))$. The ground-truth labels for the sequence are denoted as $\hat{\vvv{y}}$.\zhiyang{change y hat to y star, hat is not for gold} The score for the ground-truth label sequence is calculated as
% \begin{align*}
% S(\hat{\vvv{y}})=\sum_{i=1}^{N}{\mat{Y}_{i,\hat{\vvv{y}}_i}+\sum_{i=1}^{N-1}\mat{T}_{\hat{\vvv{y}}_i,\hat{\vvv{y}}_{i+1}}},
% \end{align*}
% where \mat{T} is a transition matrix which consists the transition scores from $\hat{\vvv{y}}_i$ to $\hat{\vvv{y}}_{i+1}$. The objective is to maximize the negative log-likelihood of the ground-truth label sequence.
% \begin{align*}
% \mathcal{L}^I(\hat{\vvv{y}})=-S(\hat{\vvv{y}})+\log{\sum_{\vvv{y}\in{\mat{Y}}}\exp{S({\vvv{y}})}},
% \end{align*}
% The representations of identified event triggers and entities are computed as the averaged token representations across the identified trigger and entity spans and are fed into two local classifiers $\textsl{FFN}^V$s to classify the event types and entity types. 
% For simplicity, we consider both event triggers and entities as a set of nodes $V$. The score vector for node $v_i$ is $\vvv{y}_{v_i}=Softmax(\textsl{FFN}^V(\frac{1}{m}\sum_d^{d+m}\vvv{w}_d))$ where $d$ is the starting index of node $v_i$ in the $W$ and m is the span size of $v_i$. The representation of each event trigger is concatenated with the representation of each entity and is fed into a local classifier $\textsl{FFN}^E$ to compute the score for argument role types. The score vector for edge $e_{ij}$ which connects node $v_i$ and node $v_j$ is $\vvv{y}_{e_{ij}}=Softmax(\textsl{FFN}^E([\frac{1}{m}\sum_d^{d+m}\vvv{w}_d,\frac{1}{n}\sum_c^{c+n}\vvv{w}_c]))$, where $d$ is the starting index of $v_i$ and $c$ is the starting index of $v_j$ in $W$ and m is the span size of $v_i$ and n is the span size of $v_j$. The objective is to minimize the cross-entropy loss:
% \begin{align*}
% \mathcal{L}^C(\hat{\vvv{y}})=-\frac{1}{|V|}\sum_{v_i\in V}\hat{\vvv{y}}_{v_i} \log{\vvv{y}_{v_i}}- \\
% \frac{1}{|E|}\sum_{e_{ij}\in E}\hat{\vvv{y}}_{e_{ij}} \log{\vvv{y}_{e_{ij}}},
% \end{align*}
% \jy{Usage of $\hat y_{v_i}$ should be unified. Right now this is one-hot vector, before it was inde vector. Likewise, $y_{v_i}$ is matrix. }
% $\hat{\vvv{y}}_{v_i}$ and $\hat{\vvv{y}}_{e_{ij}}$ are the ground truth label vectors for node $v_i$ and edge $e_{ij}$. 
% OneIE learns an additional global weight vector \vvv{u} which captures interactions across subtasks and instances. The interactions across subtasks are between entity types, event types and argument roles. For example,\zhiyang{provide one example} in an 'Attack' event, the argument with a 'LOC' entity type is unlike to have an 'Attacker' role. The interactions across instances happen between event instances. For example, the 'Defendant' in an 'Sentence' event can also be an 'Agent' in a 'Die' event. During training, the global feature $f(G)$ is collected on the current local optimal graph $G$ and the gold annotation $G'$. The objective is to make sure that the $G'$ has higher global score than $G$.
% % $\hat{\vvv{y}}_i^v$ and $\hat{\vvv{y}}_k^e$ are the ground truth label vectors for node $i$ and edge $k$. Forth, OneIE learns an additional global weight vector \vvv{u} which learns to capture the Cross-subtasks and Cross-instance interactions. During training, the global feature $f(G)$ is collected on the current local optimal graph $G$ and the gold annotation $G'$. The objective is to make sure that the $G'$ has higher global score than $G$.
% \begin{align*}
% \mathcal{L}^G(\hat{\vvv{y}})=\vvv{u}f(G)-\vvv{u}f(\hat{G}),
% \end{align*}
Finally, the combined objective for training OneIE model is
\begin{align*}
\mathcal{L}^E=\mathcal{L}^I+\mathcal{L}^C+\mathcal{L}^G.
\end{align*}



\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/overall_model.png}
    \caption{ Left is a diagram for the \stgg{}. Given an unlabeled sentence $\widetilde{W}$ and its AMR graph (green), the event extraction model computes the pseudo labels and the scoring model computes a compatibility score  to guide the self-training process. Right is the detailed description of scoring model.\minqian{argument repr, argument role repr not appear in figure but appear in legend; AMR Rel Emb and Trigger Type Emb arrows are in same color in legend} 
    }
    \label{fig:model_arch}
\end{figure*}



\section{Proposed Method}
In this section, we first explain the \selftraining{} algorithm and then present \selftraininggg{} (STGG) to alleviate the noises introduced by low-quality pseudo-labels and inject AMR knowledge into the \selftraining{} process.

\begin{table}[ht!]
%\setlength\tabcolsep{4pt}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ l | r |  }
\toprule
Symbol &   \\
\midrule
% Gradient \\
\mathcal{D}^{tr} & labeled dataset \\
\mathcal{D}^{pseu} & pseudo labeled dataset \\
$W$ & sentence in labeled dataset \\
$\mathbf{y}$ & event labels on one sentence \\
$\mathcal{W}$ & sentences in labeled dataset \\
$\hat{\mathcal{W}}$ & sentences in pseudo-labeled dataset \\
$\mathcal{Y}$ & labels in labeled dataset \\
$\hat{\mathcal{Y}}$ & pseudo labels in pseudo-labeled dataset \\
$f^e_\theta$  & OneIE model \\
$f^s_\psi$ & scoring model \\


\bottomrule
\end{tabular}
}
\end{center}
\vspace{-0.4cm}
\caption{
}
\label{tab:notation}
\end{table}
\subsection{Self-Training}
The  \selftraining{} algorithm~\cite{self-training2000,self-training2005} consists of two stages. In the first stage, an event extraction model (OneIE) is trained on a labeled dataset $ \mathcal{D}^{tr}=\{(W,\mathbf{y})\in \mathcal{W} \times \mathcal{Y}\}$ until it converges. In the second stage, the fully trained event extraction model generates pseudo labels $\tilde{\mathbf{y}}$ for event triggers, arguments, and argument roles on an unlabeled dataset $\tilde{\mathcal{W}}$. The pseudo labels are filtered by a confident threshold $s^{st}$, and pseudo labels with probabilities higher than the $s^{st}$ are collected to form the pseudo labeled dataset $ \mathcal{D}^{pseu}=\{(\tilde{W},\tilde{\mathbf{y}})\in \tilde{\mathcal{W}} \times \tilde{\mathcal{Y}}\}$. The pseudo labeled dataset is merged into the labeled dataset $\mathcal{D}^{tr}=\mathcal{D}^{tr}\cup\mathcal{D}^{pseu}$ and the event extraction model is trained on the augmented dataset. The stage two of self-training algorithm alternates between generating new pseudo labels and training the model on augmented dataset until no new confident instance can be found.
% alternates between generating pseudo labels and training the model on the union of the high-confident pseudo-labeled data and the labeled data. In the first stage of the algorithm, an event extraction model is trained on a labeled dataset $ (\mathcal{X}_L, \mathcal{Y}_L)$ until converges. Then the fully trained event extraction model generates pseudo labels $\mathcal{Y}_\mathcal{U}$ on an unlabeled dataset $\mathcal{X}_\mathcal{U}$. The pseudo-labeled instances are filtered by a confident threshold $s^{st}$ and instances with probabilities higher than $s^{st}$ are collected and form $(\hat{\mathcal{X}}_\mathcal{U},\hat{\mathcal{Y}}_\mathcal{U})$. The event extraction model is trained on $(\mathcal{X}_L, \mathcal{Y}_L)\cup(\hat{\mathcal{X}}_\mathcal{U},\hat{\mathcal{Y}}_\mathcal{U}) $ and later is used to find more confident predictions. This process ends until no new confident instance can be found.
% \zhiyang{$(\mathbf{x}, \mathbf{y})\in\mathcal{D}^{tr}$
% $(\mathbf{x}, \mathbf{y})\in\mathcal{D}^{pseu}$}
% dynamically performs self-training on the unlabeled dataset. Unlike,  ST, ST in (cite)
% \subsection{Computing Feedback}
\subsection{Self-Training with Gradient Guidance}
% Under the assumption of self-training framework, the probability (confidence) of a pseudo-label predicted by the model can reflect the correctness of the pseudo-label. Thus, high confident predictions can be added to the labeled dataset and improve the model's performance. However, this assumption breaks when the teacher model can not make reasonable predictions. As a result, without feedback and external guidance, the student model can gradually diverge on the noisy peudo-labels. To address this problem we propose STGG.
In \selftraining{}, if the event extraction model performs poorly at beginning of stage two, the predicted pseudo labels can be very noisy and inaccurate. The model iteratively trained on the inaccurate pseudo labels can accumulate errors and diverge. Thus, we propose \stgg{}, a framework that utilizes external AMR knowledge to guide the \selftraining{} process of event extraction.
As shown in Figure \ref{fig:model_arch}, \stgg{} consists of two models, an event extraction model $f^e_\theta$ and a scoring model $f^s_\psi$. Like self-training, \stgg{} consists of two stages. In the first stage, the event extraction model is trained on labeled event extraction dataset until it converges. In the second stage, the fully trained event extraction model generates event predictions on the unlabeled dataset:
\begin{align*}
\tilde{y}=\argmax_y f^e_\theta(y;\tilde{W}), \ \ \ \ \tilde{W}\sim\mathcal{W},
\end{align*}
where $\tilde{y}$ is organized by event trigger, argument and argument role predictions. Unlike \selftraining{}, \stgg{} does not simply collect high confident pseudo labels to train the model. Instead, \stgg{} utilizes an AMR graph on $\tilde{W}$ to evaluate the event predictions $\tilde{y}$. The AMR graph contains rich semantic and structural knowledge that is highly related to events. By computing the probabilities of the event predictions $\tilde{y}$ conditioned on the gold or system-labeled AMR graph, \stgg{} can estimate correctness of the predictions. 

To compute the compatibility score between an event prediction $(\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j)\in \widetilde{y}$ and an AMR graph $G^a=(V^a,E^a)$, \minqian{need to explain more on what consists an AMR graph: maybe briefly introduce in this section and add more details in appendix}we first need to align the event trigger $\widetilde{\tau}_i$ to $v^a_i\in V^a$ and $\widetilde{\varepsilon}_j$ to $v^a_j\in V^a$. Then we find the AMR path $p_{i,j}$ connecting $\widetilde{\tau}_i$ and $\widetilde{\varepsilon}_j$ by finding the shortest path between $v^a_i$ and $v^a_j$ in $G^a$.
If there is no path between $v^a_i$ and $v^a_j$, we add a new edge to connect them and assign \textit{other} as the relation. We follow \cite{AMR_IE} to perform node alignment between AMR nodes, and event triggers and arguments. Specifically, if a AMR node, and an event trigger or argument have overlaps in the text $W$, we align them. The scoring model takes the event prediction $(\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j)\in \widetilde{y}$ and its corresponding AMR path $p_{i,j}$ as input and computes a compatibility score:
\begin{align*}
c_{i,j} = f^s_\psi((\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j);p_{i,j},\widetilde{W})
\end{align*}
where $c_{i,j}$ can be interpreted as the probability of an event prediction given its corresponding AMR path and the score model's parameters. 
% \lifu{not clear, especially what does information network mean? and why perform node alignment?} %The AMR graphs can either be from manual annotations or a pre-trained AMR parser~\cite{}.
Following \selftraining{}, the event predictions with pseudo labels are passed into the event extraction model and the gradient is computed as follows:
\begin{align*}
g^{st}_{i,j} = \nabla_\theta \mathcal{L}^E\left(\widetilde{W}, (\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j);\theta\right)
\end{align*}

%Until now, the process is the same as the traditional \selftraining{} with the confident threshold $s^{st}$ set to 0. 
The direction and magnitude of the gradient $g^{st}_{i,j}$ can be incorrect due to the errors of the pseudo labels. To tackle this problem, we further use the compatibility score $c_{i,j}$ to guide the gradient by multiplying them together. However, by definition, the compatibility scores can only be non-negative which can not change the direction of the gradients for wrong predictions, thus we further design a transformation function $f^c$ to project the range of the compatibility score onto [-1,1], in our case it's a simple linear mapping as $f^c(c_{i,j})=2\times c_{i,j} -1 $ and the gradients computed by STGG for a pseudo-labeled example $\widetilde{x}$ is formulated as:
% The proposed STGG consists of two modules, an event extraction model and a scoring model. In the  self-training setting, the event extraction model is first trained on labeled dataset and then
% We follow the self-training algorithm in (cite), which unlike  ST, train the student model on each batch. Specifically, the teacher model predicts pseudo labels on a batch of unlabeled data, the confident pseudo-labeled instances are immediately used to train the student model, and the student model becomes the teacher model for the next batch. To avoid the student model diverge too much from starting point, the student model is simultaneously trained on one batch of the labeled dataset. The supervised loss works as a regularizer which shares the same goal as the $L2$ loss used in (cite). \lifu{for this paragraph, you can add two figures for comparison: one is for the  self-training, the second is for STF for which you can have an overview figure}
%Now we have all the pieces and the gradient computed by STGG for a pseudo-labeled instance $\widetilde{x}$ is formulated as:
\begin{align*}
g^{stgg} = \sum_{i,j}f^c(c_{i,j})g^{st}_{i,j},
\end{align*}
% The parameter of $f^e_\theta$ is updated as:
% \begin{align*}
% \theta_{t+1} = \theta_t - \frac{1}{B}\sum_{B}(g^{stgg}),
% \end{align*}
% where $B$ is the batch size.

o improve the efficiency of \selftraining{}, we propose to update the event extraction on every minibatch. Thus, the loss of \stgg{} is computed as follows:
\begin{align*}
\mathcal{L}^{ST} = \frac{1}{|B|}\sum_B\sum_{i,j}f^c(c_{i,j}) \cdot \\ \mathcal{L}^E\left(\widetilde{x}, (\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j);\theta\right),
\end{align*}

To avoid the model diverging, we add the supervised loss to the \selftraining{} loss and the final loss for \stgg{} is:
\begin{align*}
\mathcal{L} = \mathcal{L}^{E} + \alpha\mathcal{L}^{ST}
\end{align*}
where $\alpha$ is the combination rate.
% In the above formulation, if the event extraction model is quite confident about its prediction, the gradient $g^{(i,j)}_{st}$ for self-training is close to 0. In such case, no matter the feedback is positive or negative, it won't affect the model's parameters much because it's bounded between [-1.0,1.0]. If the EE model is not confident about its prediction, the the gradient for self-training is large. In such case, if the scoring model is not confident, the feedback is closes to 0. Hence the model's parameters won't change much either. However, if the scoring model is confident, the model's parameters move towards or in the opposite direction of the gradient based on the sign of the feedback. The step size depends on the magnitude of the gradient and the feedback.

% In the above formulation, if the event extraction model is quite confident about its prediction, the gradient $g^{st}_{i,j}$ for \selftraining{} is close to 0. In such case, the gradient guidance $f^c(c_{i,j})$ does not affect the model's parameters much because it's bounded between [-1,1]. If the event extraction model is not confident about its prediction, $g^{st}_{i,j}$ is large. In such case, if the scoring model is not confident which means $f^c(c_{i,j})$ is closes to 0, the model's parameters do not change much either. If the scoring model is confident and event extraction model is not, the model's parameters $\theta$ may move towards or in the opposite direction of the gradient based on the sign of the guidance. The step size depends on the magnitudes of both the gradient $g^{st}_{i,j}$ and the guidance $f^c(c_{i,j})$.

% The feedback is computed as $feedback=2\times score - 1$, where the $score$ reflects how good a prediction is and is bounded by $[0.0,1.0]$ which makes the $feedback$ bounded by $[-1.0,1.0]$. In our specific case
% \begin{align*}
% s_{i,j}^f=2\times C(e^a_{i,j},P_{i,j}) -1,
% \end{align*}
% where $s_{i,j}^f$ is the feedback for the predicted argument role $e^a_{i,j}$. The formulation for STF is simple and is defined as $feedback\times self\_training\_gradients$. In our case, it is $s_{i,j}^f\times \mathcal{G}^{st}_{i,j}$, where $\mathcal{G}^{st}_{i,j}$ is the self-training gradient for $e^a_{i,j}$. 
\subsection{Scoring Model} \label{sec:score_model_method}
The scoring model aims to estimate the correctness of the prediction of each candidate trigger and argument. Inspired by the coherence between the event structures and AMR graphs, we propose to leverage the AMR graph to better capture the semantic relation between the candidate trigger and argument in our scoring model.

Given an input sentence $W$ and its corresponding AMR graph $G^a=(V^a,E^a)$, each node $v^a_i\in V^a$ can be mapped to a word in $W$. Thus, we first apply a language model encoder \cite{bert,roberta} to compute the contextual representations for the sequence of tokens in $W$ and then use them to initial the representation $\vvv{h}^v_i$ of each node $v^a_i$. For each AMR relation $e^a_{i,j}$, we randomly initialize a vector representation $\vvv{h}^e_{i,j}$ for $e^a_{i,j}$, and use $\mat{E}^{rel}$ to denote the embedding matrix of all AMR relations. Given a predicted trigger $\widetilde{\tau}_i$ and argument $\widetilde{\varepsilon}_j$, we identify their corresponding nodes $v^a_i$ and $v^a_j$ in $G^a$ by node alignment following~\cite{AMR_IE}, and utilize the Breadth First Search (BFS) to find the shortest path $p_{i,j}$ that connects $v^a_i$ and $v^a_j$ in $G^a$. Then we concatenate a virtual event type node, the path and a virtual argument role node as an overall sequence $\mat{H}^{init}_{i,j}=[\vvv{h}^t_i,\vvv{h}^v_i, \vvv{h}^e_{i,i+1}, \vvv{h}^v_{i+1},...,\vvv{h}^v_{j-1}, \vvv{h}^e_{j-1,j}, \vvv{h}^v_j, \vvv{h}^a_{i,j}]$, where both the event type representation $\vvv{h}^t_i$ and argument role representation $\vvv{h}^a_{i,j}$ are drew from the randomly initialized event embedding matrix $\mat{E}^{tri}$ and argument role embedding matrix $\mat{E}^{arg}$. We also add token type embeddings to $\mat{H}^{init}_{i,j}$ to help the model understand the input types which are AMR node, AMR relation, event trigger type, and argument role type.

In order to estimate the correctness of the predicted event trigger and candidate argument, we further design a \textit{self-attention layer}~\cite{transformer} over $\mat{H}^{init}_{i,j}$ to learn a new contextual representation for each node or relation in the AMR path:
\begin{align*}
 \mat{H}^{final}_{i,j}= \textit{self-attention}(\mat{H}^{final}_{i,j})\times M,
\end{align*}
where $M$ denotes the number of attention layers.

We compute an overall vector representation from $\mat{H}^{final}_{i,j}$ as $\vvv{h}^{final}_{i,j}$ based on average-pooling and feed it into a \textit{linear-layer} and a \textit{Sigmoid} function to compute a probability $c_{i,j}$, indicating the correctness of the predicted event trigger and argument. We optimize the scoring model based on the binary cross-entropy objective:
\begin{align*}
%  c_{i,j} = 
%  \mathcal{L}^s= \text{BCE}\left(y_i,f^s_\psi\left((\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j);p_{i,j}\right)\right),
 \mathcal{L}^s= \text{BCE}\left(y_{i,j}, c_{i,j}\right),
\end{align*}
where $y_{i,j}$ is a binary label which indicates whether the argument role is correct ($y_{i,j}=1$) or not ($y_{i,j}=0$). During training, we have the ground-truth labels as positive training instances and we swap the labels of argument roles in positive training instances with randomly sampled incorrect labels to create negative training instances. %All three event extraction datasets we used do not have AMR annotations. Thus, following~\citep{AMR_IE}, we run an AMR parser~\citep{transformer_amr_parser} trained on AMR 3.0 to generated system-labeled AMR graphs.

%We propose to leverage the \textit{self-attention layer} \cite{transformer} to achieve full interaction between AMR relations and nodes, and between the AMR path and the event prediction.

%. Then we concatenate the node and edge representations on $p_{i,j}$ to form $\mat{H}^{init}_{i,j}=[\vvv{h}^v_i, \vvv{h}^e_{i,i+1}, \vvv{h}^v_{i+1},...,\vvv{h}^v_{j-1}, \vvv{h}^e_{j-1,j}, \vvv{h}^v_j]$. To represent the event prediction $(\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j)$, we randomly initialize the embedding matrices $\mat{E}^{tri}$ for event trigger types $L^t$ and $\mat{E}^{aug}$ for argument role types $L^a$ and draw $\vvv{h}^t_i$ from $\mat{E}^{tri}$ as the event type representation and draw $\vvv{h}^a_i$ from $\mat{E}^{aug}$ as the argument role type representation. To inform the scoring model about the event prediction, we concatenate the event representation to $\mat{H}^{init}_{i,j}$: $\mat{H}^{init}_{i,j}=[\vvv{h}^t_i,\vvv{h}^v_i, \vvv{h}^e_{i,i+1}, \vvv{h}^v_{i+1},...,\vvv{h}^v_{j-1}, \vvv{h}^e_{j-1,j}, \vvv{h}^v_j, \vvv{h}^a_{i,j}]$. We also add token type embeddings to $\mat{H}^{init}_{i,j}$ to help the model understand the input types. We propose to leverage the \textit{self-attention layer} \cite{transformer} to achieve full interaction between AMR relations and nodes, and between the AMR path and the event prediction.

% In this section, we explain the design and training process of the self-attention~\citep{transformer} based scoring model. The goal of the scoring model $f^s_\psi$ is to effectively utilize the the AMR graph to estimate the probability of an event prediction. The proposed model architecture, as shown in Figure~\ref{fig:model_arch}, can capture the interaction between AMR nodes and relations, and induce the semantic and structure knowledge from the AMR graph.
% that computes the compatibility score between a predicted triple of (event trigger $(\tau_i)$, argument role $(a_{i,j})$, argument $(\varepsilon_j)$) and it's corresponding AMR path $p_{i,j}$, the shortest path between $\tau_i$ and $\varepsilon_j$ in the AMR graph $G^{a}=(V^a,E^a)$.

% of an argumnet role $e^a_{i,j}$ conditioned on an event trigger and entity pair$(\tau_i,\varepsilon_j)$, and an AMR path $P_{i,j}$ which is a subgraph of the AMR graph $G^a=(V^a,E^a)$. 
% We propose the sequence scoring model to address the sparse interaction problem inherently in the graph-based model and better use the AMR relation information.
% The AMR graph $G_a$ is obtained by the transformer-based AMR parser \cite{transformer_amr_parser} pretrained on AMR 3.0 (cite). 
% In some cases, one can easily identify the correspondence between and argument role type and the AMR path. However, unlike the information network \cite{information_netwroks}, in which the triggers and entities are always directly connected, the AMR graph can have multi-hop relations and additional nodes between triggers and entities. Thus, the rule based scoring method is not applicable and we develop a machine-learning model to extract the abstraction of the AMR path. 

% \lifu{make the following as a paragraph}
% \paragraph{Representation Initialization}
% In the AMR graph $G^a=(V^a,E^a)$, each node $v^a_i\in V^a$ can be located to a span in the text $W$. Thus, we leverage the language encoder \cite{bert,roberta} to compute the contextualized word representations and take the averaged representations across a span as the initial representation $\vvv{h}^v_i$ for the corresponding AMR node $v^a_i$. We randomly initialize the embedding matrix $\mat{E}^{rel}$ for a predefined set of AMR relations and the initial representation of the relation $\vvv{h}^e_{i,j}$ on edge $e^a_{i,j}\in E^a$ is drawn from $\mat{E}^{rel}$.
% The relation on an edge $e^a_{i,j}$ is assigned from a predefined set of AMR relations $R^a$. We randomly initialize the embedding matrix $\textbf{E}^a$ for $R^a$ and for an edge $e^a_{i,j}$, it's embedding is drawn from $\textbf{E}^a$ and denoted as $\vvv{h}^e_{i,j}$.  
% To calculate the initial node representations $H^{node}$ for $V_a$, we align $V_a$ to the phrases in $\textbf{\textit{w}}$ and take the averaged contextualized word representations across the phrase spans. The edge representations $H^{edge}$ are randomly initialized. In addition, We followed\lifu{make all the tense consistent} AMR-IE\lifu{add reference} to perform Node Alignment\lifu{why they are capitalized?} which maps the nodes from information networks to AMR graph by leveraging their span offsets in the text. For triggers and entities that do not appear in AMR graph, we add them and add additional edges\lifu{what are the edge labels?} to connect them to their nearest neighbours.
% \subsection{Graph-Based Scoring Model} \\
% This graph-based scoring model is a strong baseline derived from AMR-IE \cite{AMR_IE}. Same as AMR-IE, we use Graph Attention Networks (GATs) \cite{GAT} to perform Attention Based Message Passing. On each layer, the triggers and entities aggregate neighbouring information based on attention scores computed by the node and edge features.  
% \begin{align*}
% \alpha_{i,j}^l=\frac{\exp{(\sigma( [\textbf{W}h_i^l,\textbf{W}_eh^e_{i,j},\textbf{W}h_j^l]) )}}{\sum_{k\in \mathcal{N}_i}\exp{(\sigma( [\textbf{W}h_i^l,\textbf{W}h^e_{i,k},\textbf{W}h_k^l]) )}},
% \end{align*}
% $\mathcal{N}_i$ is the set of neighbours for node $i$, $\textbf{W}$ and $\textbf{W}_e$ are trainable parameters, $h^l_i$ is the representation for node $v_i$ on layer $l$, and $h^e_{i,j}$ is the representation for edge $e_{i,j}$. The aggregated information is $h'=\sum_{j \in \mathcal{N}_i}a_{i,j}^l h_i^l$ and the representation on layer $l+1$ is $h^{l+1}=h^l+\gamma h^l'$, where $\gamma$ controls the level of message passing. The representation $h^L_i$ on final layer contains the structure information embedded in the AMR graph. 
% \paragraph{Computing the Contextualized Representations for an AMR Path} \\
% Given the predicted trigger $\widetilde{\tau}_i$ and argument $\widetilde{\varepsilon}_j$, we identify their corresponding nodes $v^a_i$ and $v^a_j$ in $G^a$ by node alignment \cite{AMR_IE}, and utilize the Breadth First Search (BFS) to find the shortest path $p_{i,j}$ that connects $v^a_i$ and $v^a_j$. Then we concatenate the node and edge representations on $p_{i,j}$ to form $\mat{H}^{init}_{i,j}=[\vvv{h}^v_i, \vvv{h}^e_{i,i+1}, \vvv{h}^v_{i+1},...,\vvv{h}^v_{j-1}, \vvv{h}^e_{j-1,j}, \vvv{h}^v_j]$. 
% To represent the event prediction $(\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j)$, we randomly initialize the embedding matrices $\mat{E}^{tri}$ for event trigger types $L^t$ and $\mat{E}^{aug}$ for argument role types $L^a$ and draw $\vvv{h}^t_i$ from $\mat{E}^{tri}$ as the event type representation and draw $\vvv{h}^a_i$ from $\mat{E}^{aug}$ as the argument role type representation. To inform the scoring model about the event prediction, we concatenate the event representation to $\mat{H}^{init}_{i,j}$: $\mat{H}^{init}_{i,j}=[\vvv{h}^t_i,\vvv{h}^v_i, \vvv{h}^e_{i,i+1}, \vvv{h}^v_{i+1},...,\vvv{h}^v_{j-1}, \vvv{h}^e_{j-1,j}, \vvv{h}^v_j, \vvv{h}^a_{i,j}]$. We also add token type embeddings to $\mat{H}^{init}_{i,j}$ to help the model understand the input types.
% We propose to leverage the \textit{self-attention layer} \cite{transformer} to achieve full interaction between AMR relations and nodes, and between the AMR path and the event prediction.
% \begin{align*}
%  \mat{H}^{final}_{i,j}= \textit{self-attention}(\mat{H}^{final}_{i,j})\times M,
% \end{align*}
% We pool the sequence representations $\mat{H}^{final}_{i,j}$ to form $\vvv{h}^{final}_{i,j}$ and pass it through a \textit{linear-layer} and the \textit{Sigmoid} function to compute a probability $c_{i,j}$.
% Finally, the loss is computed as:
% \begin{align*}
%  \mathcal{L}^s= \text{BCE}\left(y_i,f^s_\psi\left((\widetilde{\tau}_i, \widetilde{a}_{i,j}, \widetilde{\varepsilon}_j);p_{i,j}\right)\right),
% \end{align*}
% where $y_i$ is a binary label which indicates either the event prediction is correct or not. During training, we have the ground-truth event annotations as positive training instances and we swap the event labels in positive training instances with randomly sampled incorrect labels to create negative training instances. All three event extraction datasets we used do not have AMR annotations. Thus, following~\citep{AMR_IE}, we run an AMR parser~\citep{transformer_amr_parser} trained on AMR 3.0 to generated system-labeled AMR graphs.
% Then we collect the node representations $M^{node}$ for $V^p$ from $H^{node}$ and edge representations $M^{edge}$ for $E^p$ from $H^{edge}$
% \lifu{these math symbols are messy and the main reason is they are not indicative to their meanings. Try to have a set of math symbols with clear annotations}. 
% We then concatenate the node and edge representations to form a sequence $H^{path}$. To inform the scoring model of the trigger, entity and argument role types, we have randomly initialized embeddings for all types and concatenate the trigger, entity and argument role embeddings to $H^{path}$, which now becomes $[trigger\_type\_emb, AMR\_path\_repr, \\ entity\_type\_emb,arg\_role\_type\_emb]$. We further add position embeddings $H^{emb}$ and token type embeddings $H^{type}$ to allow the model to understand the order of the sequence and distinguish AMR nodes, AMR relations, and EE labels. Then $H^{path}$ is passed into self-attention layers \cite{transformer} to capture the interaction between nodes, edges and labels and learn better representations. The final representations are $H^{f}=self\_attention\_layers(H^{path})$.
% We further concatenate the trigger type $e^t$ and argument role type $e^a$ to the end of $H^{path}$. 
% To capture the interaction between nodes and edges and learn semantic and structure knowledge on the AMR path, we apply the self-attention-layer from \cite{transformer} to $H^{path}$.
% \paragraph{Computing the Compatibility Score} \\
% We define the compatibility score as $C(e^a_{i,j},P_{i,j})=P(e^a_{i,j}|(\tau_i,\varepsilon_j),P_{i,j};W^s)$, where $W^s$ is the trainable parameters. We employ a simple linear-layer $f^s(\cdot)$ as the classifier which takes in the pooled representation of the AMR path $\textbf{h}^p\in H^{f}$, the argument role type representation $\textbf{h}^a\in H^{f} $, and output the score $C(e^a_{i,j},P_{i,j})=sigmoid(f^s([\textbf{h}^p,\textbf{h}^a]))$, where $C(e^a_{i,j},P_{i,j}) \in [0.0,1.0]$. During training, we apply binary-cross-entropy loss
% \begin{align*}
% \mathcal{L}^C(e^a_{i,j})=-(\mathbbm{1}[e^a_{i,j}=y^a_{i,j}]*\log{C(e^a_{i,j},P_{i,j})}\\
% +(1-\mathbbm{1}[e^a_{i,j}=y^a_{i,j}])*\log{1-C(e^a_{i,j},P_{i,j})}),
% \end{align*}
% where $\mathbbm{1}[]$ is the indicator function and $y^a_{i,j}$ is the gold argument role label. For each instance, we also create negative instances by assigning all other incorrect argument role types. 
% We don't apply softmax to the labels, because we don't want the label to exclude each other. Our prediction is not a single label but how good the label is. 
% % Sometimes a wrong label is also reasonable as a prediction but just not as good as the correct one. In such case, our score model will compute a low but reasonable score which can help the student model to understand the latent connections between labels. 
% The predicted probabilities contain richer information comparing to a one-hot distribution.



% We model the scoring problem as an entailment problem. Given $\tau_i,\varepsilon_j$ and $G_a$, the score model aims to predict $P(e^a_{i,j}|(\tau_i,\varepsilon_j),G_a;W^s)$, where $W^s$ is the trainable parameters. We employ a simple linear-layer $f^s(\cdot)$ as the classifier which takes in the pooled representation of the AMR path $\textbf{h}^p$, the embedding $\textbf{h}^a$ of an argument role type, and the embedding $\textbf{h}^t$ of an event trigger type and output a score $s^c\in [0.0,1.0]$. There are many strategies to feed $\textbf{h}^p$, $\textbf{h}^a$ and $\textbf{h}^t$ into the classification layer. For Graph-based model we simply concatenate them. For Seq-based model, we concatenate the $\textbf{h}^a$ and $\textbf{h}^t$ to the end of $H^{path}$ before passing it to the self-attention layers. With the self-attention layers and token type embeddings, the pooled AMR path $\textbf{h}^p$ already contains the label information. During training, for each instance, we create negative instances by assigning all other incorrect argument role types. We don't apply softmax to the labels, because we don't want the label to exclude each other. Our prediction is not a single label but how good the label is. Sometimes a wrong label is also reasonable as a prediction but just not as good as the correct one. In such case, our score model will compute a low but reasonable score which can help the student model to understand the latent connections between labels. The predicted probabilities contain richer information comparing to a one-hot distribution. To achieve this goal, we employ the binary-cross-entropy as the objective. In addition, we want the correct label to have high probability than the incorrect labels, thus we add additional hinge-loss to push the probability of correct label higher. We have a hyperparameter $\beta$ to combine the loses. One can view our combined loss as a soft version of cross-entropy loss where $\beta$ decides how much the probability of correct label squeezes the probabilities of other labels.\\


% \subsection{The Dynamics between Gradients and Feedback}
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/model_arch.jpeg}
%     \caption{The overall schema of self-training with feedback. The text is passed into the teacher model to produce the pseudo labels. Both the text and the AMR annotation are passed into the text encoder to compute the node representation for the AMR graph. Then the nodes in the predicted information networks are aligned with the nodes in AMR graph. The identified AMR path and event trigger, entity and argument role are passed into the score model to predict a compatibility score, which is later used as feedback for guide the training of the student model.     
%     }
%     \label{fig:model}
% \end{figure}
% \subsection{Self-Training}
% The  self-training algorithm (cite) alternates between a teacher and a student model. During training, the teacher model is trained on labeled data $ \mathcal{X}$ and generate pseudo labels on unlabeled dataset $\mathcal{U}$. The confident pseudo-labeled instances $\hat{\mathcal{U}}$ are added to $ \mathcal{X}$. The student model is trained on $\mathcal{X}\cup\hat{\mathcal{U}}$ and the student model becomes the new teacher model to find more confident instances. This process ends until no new confident instances can be found. We follow the self-training algorithm in (cite), which unlike  ST, train the student model on each batch. Specifically, the teacher model predicts pseudo labels on a batch of unlabeled data, the confident pseudo-labeled instances are immediately used to train the student model, and the student model becomes the teacher model for the next batch. To avoid the student model diverge too much from starting point, the student model is simultaneously trained on one batch of the labeled dataset. The supervised loss works as a regularizer which shares the same goal as the $L2$ loss used in (cite).

% % dynamically performs self-training on the unlabeled dataset. Unlike,  ST, ST in (cite)
% % \subsection{Computing Feedback}
% \subsection{Guide Self-Training with Feedback}
% The feedback is computed as $feedback=2\times score - 1$, where the $score$ reflects how good a prediction is and is bounded by $[0.0,1.0]$ which makes the $feedback$ bounded by $[-1.0,1.0]$. In our specific case
% \begin{align*}
% s_{i,j}^f=2\times C(e^a_{i,j},P_{i,j}) -1,
% \end{align*}
% where $s_{i,j}^f$ is the feedback for the predicted argument role $e^a_{i,j}$. The formulation for STF is simple and is defined as $feedback\times self\_training\_gradients$. In our case, it is $s_{i,j}^f\times \mathcal{G}^{st}_{i,j}$, where $\mathcal{G}^{st}_{i,j}$ is the self-training gradient for $e^a_{i,j}$. 
% when the predicted probability is higher than $0.5$, the EE model will have a positive feedback and 
% Given a predicted triple of an argument role $e^a_i$, and the corresponding AMR path $S_{a}$, the score model compute a compatibility score $s_i^c=P(|\tau_i,)$ between $S_a$ and $e^a_i$. Follow \cite{ConstrainedSRL}, we compute the feedback as $s_i^f=2\times s_i^c-1$ and $s_i^f\in [-1,1]$. 
% When $s_i^c>0.5$, $s_i^g$ is positive and the score model support current prediction. will follow the direction of the gradient computed from the pseudo label  by the magnitude of $s_i^g$ when $s_i^c>0.5$, $s_i^g$ is positive

% \paragraph{Event Trigger feedback} Since there is no strong label correlation between AMR nodes and event triggers, we can not directly compute feedback from the scoring model. Instead, we take the averaged the feedback of argument roles around the trigger as its feedback, 
% $s_{i}^f=\frac{1}{|\mathcal{N}_i|}\sum_{j\in \mathcal{N}_i}s_{i,j}^f$.
% The aggregated feedback $s_{i}^f$ can provide meaningful information because when the scoring model evaluates the predicted argument role, it also takes the event trigger type into account. Our assumption is that if the predicted event trigger is incorrect, the compatibility scores of all the argument roles around it are affected and drop lower.
% \subsection{Guide Self-Training with Feedback}
% Our training schema is developed on online self-training.
% Unlike  self-training which only utilizes confident predictions, STF utilize all predicted pseudo labels for training. 
% The formulation for STF is simple and is defined as $feedback\times self\_training\_gradients$. In our specific case, it is $s_{i,j}^f\times \mathcal{G}^{st}$, where $\mathcal{G}^{st}_{i,j}$ is the self-training gradient for $e^a_{i,j}$. 
% As one may notice this gradient is only computed on the argument roles classification task. However, this gradient will back-propogate into the language model. Thus, we need the supervised loss to adapt other parameters to the change of the language model.


% Since the feedback are conditional on labels, the gradient $\mathcal{G}^s$ for self-training is only computed on the classification tasks. The gradient $\mathcal{G}^s$ is calculated on the encoder as well, thus we add the supervised loss as a regularizer and it keeps updating other parameters of the model to adapt the changes in the encoder. After computing $\mathcal{G}^s$, we perform $\mathcal{G}^s \times s^f$. This way the direction and magnitude of the gradient are controlled by the feedback.
% If the score model predicts probability close to 1.0, the student model take a large step follow the direction of the gradient computed by the pseudo labels and if the predicted probability is close to 0.0, the the student model takes a large step in the opposite direction of the gradient. Unlike ST which can only take the confident positive instances for training, STF can utilize negative instance as well and allows the algorithm to use the pseudo labeled instances more efficiently.


% \subsection{Additional Heuristics}
% To better capture the interaction of the EE model and score model, we propose additional heuristics which are defined as follows. The confidence $c_e$ of EE predicted label $y$ is same as the probability $p_e \in [0,1]$ computed by the model, and the confidence of score model is calculated as $c_s=\lvert p_s-0.5 \rvert*2$ where $p_s \in [0,1]$ is the probability for $y$. $\tau \in [0,1]$ is a hyperparameter. The feedback $f \in [0,1]$ is calculated as follow:
% \begin{itemize}
%   \item If $p_s > 0.5$, $f=2*p_s-1$,  
%   \item If $p_s < 0.5$ and $c_s-c_e>\tau$, $f=2*p_s-1$  
%   \item If $p_s < 0.5$ and $c_e-c_s>\tau$, $f=0$ 
%   \item If $p_s < 0.5$ and $\lvert c_e-c_s\rvert<\tau$, $f=p_s+p_e-1$ 
% \end{itemize}
% We discuss the necessity of the human defined rules in section cite(6.4). 

% \subsection{Ways of Using feedback}
% {\large 1. Directly use prediction from translation} \\
% {\large 2. use translation to guide the gradient of self-training} \\
% {\large 3. only use translation to reject bad self-training instances} \\
% {\large 4. only use translation to with heuristics to guide self-training} \\

% \subsection{Final Objective} 
% The gradients $\mathcal{G}^{st}_{i,j}$ are only computed on the argument roles classification task but are back-propogated into the language model. Thus, we need the supervised loss to adapt other parameters to the change of the language model. The final objective for STF is a combination of supervised loss $\mathcal{L}^S$, self-training loss $\mathcal{L}^U$, and feedback $s^f$. As mentioned in Section (ref 4.1), the supervised loss also works as a regularizer and the self-training loss encourages the model to explore more space and achieve better generalizability. The final experession of the total loss is
% \begin{align*}
% \mathcal{L}=\mathcal{L}^S+\alpha s^f \mathcal{L}^U,
% \end{align*}
% where the $\alpha$ is the combine ratio. 




